Cooperative Multi-Agent Path Finding: Beyond Path Planning and Collision Avoidance

We introduce the Cooperative Multi-Agent Path Finding (Co-MAPF) problem, an extension to the classical MAPF problem, where cooperative behavior is incorporated. In this setting, a group of autonomous agents operate in a shared environment and have to complete cooperative tasks while avoiding collisions with the other agents in the group. This extension naturally models many real-world applications, where groups of agents are required to collaborate in order to complete a given task. To this end, we formalize the Co-MAPF problem and introduce Cooperative Conflict-Based Search (Co-CBS), a CBS-based algorithm for solving the problem optimally for a wide set of Co-MAPF problems. Co-CBS uses a cooperation-planning module integrated into CBS such that cooperation planning is decoupled from path planning. Finally, we present empirical results on several MAPF benchmarks demonstrating our algorithm's properties.

==> algorithms/get_next_meeting.tex <==
\begin{algorithm}[ht]
\caption{Get next meeting}
\label{alg:next_meeting}
\begin{algorithmic}[1]
\State \textbf{Input:} Meetings table $\meetingtable{i}{}$, meeting of task $\task{i}$, $\argument{\meetinglocation{i}, \meetingtime{i}{}}$

\State \textbf{Returns:} The next best meeting for task $\task{i}$

\State $\meetingtime{i}\argument{\meetinglocation{i}} = \meetingtime{i}\argument{\meetinglocation{i}} + 1$ \Comment{earliest meeting time in $\meetinglocation{i}$}
 
\State Update $\meetingtable{i}{}\argument{v}$ \Comment{update the cost}

\State Return the lowest cost meeting in $\meetingtable{i}{}$

\end{algorithmic}
\end{algorithm}
